Decomposition-based Hierarchical Task Allocation and Planning for Multi-Robots under Hierarchical Temporal Logic Specifications

Past research into robotic planning with temporal logic specifications, notably Linear Temporal Logic (LTL), was largely based on a single formula for individual or groups of robots. But with increasing task complexity, LTL formulas unavoidably grow lengthy, complicating interpretation and specification generation, and straining the computational capacities of the planners. A recent development has been the hierarchical representation of LTL~\cite{luo2024simultaneous} that contains multiple temporal logic specifications, providing a more interpretable framework. However, the proposed planning algorithm assumes the independence of robots within each specification, limiting their application to multi-robot coordination with complex temporal constraints. In this work, we formulated a decomposition-based hierarchical framework. At the high level, each specification is first decomposed into a set of atomic sub-tasks. We further infer the temporal relations among the sub-tasks of different specifications to construct a task network. Subsequently, a Mixed Integer Linear Program is used to assign sub-tasks to various robots. At the lower level, domain-specific controllers are employed to execute sub-tasks. Our approach was experimentally applied to domains of navigation and manipulation. The simulation demonstrated that our approach can find better solutions using less runtimes.

==> introduction.tex <==
\section{Introduction}
The field of temporal logic planning has seen rapid expansion in recent years, which can manage a more diverse range of tasks beyond the typical point-to-point navigation, encompassing temporal objectives as well. These tasks involve sequencing or coverage~\cite{fainekos2005temporal}, data collection~\cite{guo2017distributed}, intermittent communication~\cite{kantaros2018distributed}, manipulation~\cite{he2015towards}  and persistent surveillance~\cite{leahy2016persistent} among others. For a comprehensive review of formal specifications and synthesis techniques applicable to robotic systems, refer to~\cite{luckcuck2019formal}. Here, we focus on Linear Temporal Logic (LTL) specifications~\cite{pnueli1977temporal}. However, to the best of knowledge, except for~\cite{luo2023simultaneous}, all LTL formulas, regardless of whether they are assigned locally or globally, are in the flat structure, meaning a single LTL formula specifies the behavior of an individual robot or a team of robots. These flat formulas tend to become cumbersome and difficult to interpret for complex tasks. Studies~\cite{tenenbaum2011grow} suggest that humans prefer hierarchical task specification, which improves interpretability of planning and execution, making it easier to identify ongoing work and conveniently adjust unfeasible parts without affecting other components. 

In our prior work \cite{luo2023simultaneous}, we introduced a hierarchical and interpretable structure for LTL specifications, consisting of various levels of flat specifications that enhance computational efficiency. A bottom-up planning approach was developed for simultaneous task allocation and planning. While this method is efficient, it operates under the assumption that  tasks with temporal dependencies within a flat specification is allocated to a single robot, hence robots can work independently, limiting its application in scenarios that require cooperation among multiple robots.

In this work, we have developed a hierarchical framework capable of addressing multi-robot coordination under hierarchical temporal logic specifications. This framework starts at the top level by breaking down each flat specification into smaller sub-tasks. These sub-tasks are then organized into a {\it task network}, where we deduce the temporal relationships between them. Subsequently, we use a Mixed Integer Linear Programming (MILP) approach to assign these sub-tasks to various robots. At the lower level, we implement domain-specific planning methods to carry out these sub-tasks.

In this work, our contributions are outlined as follows:
\begin{enumerate}
\item A computationally efficient hierarchical framework for hierarchical LTL specifications has been developed;
\item The effectiveness of hierarchical method  for navigation and manipulation tasks in multi-robot systems has been demonstrated.
\end{enumerate}



==> literature.tex <==
\section{Related Work}

In the most research that centered on multi-robot systems, LTL tasks are either assigned {\it locally} to individual robots within a team~\cite{guo2015multi,tumova2016multi,yu2021distributed,bai2022hierarchical}, or a {\it global} LTL specification is used to capture the collective behavior of all robots. In the latter approach, tasks can either be explicitly assigned to each robot, as in~\cite{loizou2004automatic,smith2011optimal,saha2014automated,kantaros2020stylus,luo2019transfer,luo2021abstraction}, or task allocation is considered without specific assignments, as in~\cite{shoukry2017linear,schillinger2018simultaneous,sahin2019multirobot, leahy2021scalable,luo2022temporal,li2023fast}. 
 

Global temporal logic specifications that do not explicitly assign tasks to robots generally require decomposition to derive the necessary task allocation. This decomposition can be accomplished in three primary ways: The most common method, utilized in works such as~\cite{schillinger2018simultaneous,luo2019transfer,camacho2019ltl,luo2022temporal,liu2024time}, involves decomposing a global specification into multiple tasks, which leverages the transition relations within the automaton, which is the graphical representation of an LTL formula. As demonstrated in~\cite{shoukry2017linear,sahin2019multirobot}, the second approach builds on Bounded Model Checking (BMC) methods~\cite{biere2006linear} to create a Boolean Satisfaction or Integer Linear Programming (ILP) model, which simultaneously addresses task allocation and implicit task decomposition in a unified formulation. Another method, proposed by~\cite{leahy2022fast}, directly interacts with the syntax tree of LTL formulas, which segments the global specification into smaller, more manageable sub-specifications. 


 
% \subsection{Hierarchical Task Models}
% Hierarchical reasoning enhances human understanding of the world~\cite{tenenbaum2011grow, kemp2007learning}. In classical AI planning, researchers have crafted various task models reflecting hierarchical structures by employing procedural domain control knowledge~\cite{wilkins2014practical}. These models have proven to be superior to flat models in terms of interpretability and efficiency, largely due to the significant reduction in the search space for a plan. Hierarchical Task Network (HTN)~\cite{georgievski2015htn}, a commonly used task model in classical AI, exemplifies this. It presents a hierarchy of tasks, each of which can be executed if it's primitive, or broken down into finer sub-tasks if it's complex. The planning process begins with decomposing the initial task network and continues until all compound tasks are decomposed, leading to a solution. The resulting plan comprises a set of primitive tasks applicable to the initial world state. Owing to its expressive capacity, HTN has been implemented in the robotic planning~\cite{weser2010htn}.
% % There are other hierarchical models such as \texttt{AND/OR} graphs~\cite{de1990and} and sequential/parallel graphs~\cite{cheng2021human}. 

% Research combining hierarchical task models with LTL includes studies that use LTL to express temporally extended preferences over tasks and sub-tasks in HTN~\cite{baier2009htn}, as well as research into the expressive power of HTN in combination with LTL~\cite{lin2022expressive}.  However, despite the widespread use of hierarchical task models in classical AI planning, it's intriguing to note the lack of specification hierarchy in temporal logic robotic planning. Our work differs from these studies as we follow an inverse direction; instead of integrating LTL into HTN to express preferences or constraints of tasks, we incorporate HTN into LTL, allowing for hierarchical structures within multiple LTL formulas.

% Depending on the structure of the models, they can be categorized as flat models, such as a plan network~\cite{levine2014concurrent}, or hierarchical models, such as and/or graphs~\cite{de1990and}. Hierarchical models have shown superiority over flat models for human-robot collaboration, because levels of abstraction in hierarchical models are close to human intuitions, which can help predict actions of human and plan predicable actions of the robot.


% Hierarchical task models surpass the flat models in the fields of human-robot collaboration in three ways. First, hierarchical task models provide more intuitive abstractions of the task for the robots, which can help improve the human-robot communication about the intermediate goals of the task~\cite{mori2002ctte, garland2001learning}.
% Second, since humans follow the hierarchical abstractions when accomplishing a task, hierarchical task models can help predict the human’s actions~\cite{qi2017predicting,pei2011parsing}. Finally, it has been found that such hierarchical abstractions can be learned remarkably fast from relatively little data compared with what is needed for learning at lower levels due to overhypotheses~\cite{tenenbaum2011grow, kemp2007learning}.


% In the field of formal-logic-based control, hierarchy appears in abstracting out the environment or dynamics of agent~\cite{kloetzer2007temporal, fainekos2007hierarchical}. A hierarchical control system consists of (at least) two layers. The first layer consists of a coarse (and simple) model of the plant. A controller is designed so that this abstraction meets the specification of the problem. The control law is then refined to the second layer which consists of a detailed model of the plant.
% \begin{figure}[!t]
%     \centering
%     \includegraphics[width=\linewidth]{fig/desktop.png}
%     \caption{The sequential/parallel task model for a desktop assembly task\cite{cheng2021human}.}
%     \label{fig:desktop}
% \end{figure}


==> short_formulation.tex <==
\section{Problem Definition}\label{sec:problem}
\subsection{Transition system}\label{sec:ts}
Consider a discrete workspace containing $l\in \mathbb{N}^+$ labeled regions, where each region can span multiple cells, and denote by $\mathcal{L}=\{\ell_k\}_{k\in[l]}$ the set of regions, where $[l]$ is the shorthand notation for $\{1, \ldots, l\}$. We also assume that the workspace contains obstacles which do not overlap with  regions.   A  cell  is {\em region-free} if it does not belong to any region, and a path   connecting two regions  is {\em label-free} if it only passes through region-free cells. We represent the workspace by a graph $E = (S, \to_E)$ where $S$ is the finite set of free cells and $\to_{E} \subseteq S \times S$ captures the adjacency relation.

 Given the workspace $E$, we consider a team of $n$ heterogeneous robots. We assume that these robots are of $m$ different types  and every robot belongs to exactly one type. Let $\mathcal{K}_j, j\in[m]$,  denote the set that  collects all robots of type $j$, so that $\sum_{j\in [m]} |\ccalK_j| = n$ and $\ccalK_{j} \cap \ccalK_{j'} = \emptyset$ if $j \not= j'$, where $|\cdot|$ is the cardinality of a set. We collect all $n$ robots in the set $\ccalR$, i.e., $\ccalR = \{\ccalK_j\}_{j\in [m]}$. Finally, we use $[r,j]$ to represent robot $r$ of type $j$, where $r\in \ccalK_j, j\in [m]$. To model the motion  of robot $[r,j]$ in the workspace, we define a transition system (TS) for this robot as follows.

\begin{defn}[TS]\label{def:ts}
  {A transition system for robot $[r,j]$ is a tuple $\textup{TS}_{r,j} = (S, s_{r,j}^0, \to_{r,j}, \Pi_{r,j}, L_{r,j})$ where: (a) $S$ is the set of free cells; (b) $s_{r,j}^0$ is the initial location of robot $[r,j]$; (c) $\to_{r,j} \subseteq \to_{E}  \bigcup \cup_{s_{r,j}\in S} \{(s_{r,j},s_{r,j})\} $ is the transition relation that allows the robots to remain idle or move between cells;} (d) $\Pi_{r,j} = \cup_{k\in [l]}\{p_{r,j}^k\} \cup \{\epsilon\}$ where the atomic proposition $p_{r,j}^{k}$ is true if robot $[r,j]$ is at region $\ell_k$ and $\epsilon$ denotes the  empty label; and (e) $L_{r,j}: S \to {\Pi_{r,j}} $ is the labeling function that returns the atomic proposition  satisfied at location $s_{r,j}$.
\end{defn}

Next we define the  product transition system (PTS), which captures all possible combinations of robot behaviors.
\begin{defn}[PTS]\label{def:pts}
{ Given $n$ transition systems \textup{TS}$_{r,j} = (S, s_{r,j}^0, \to_{r,j}, \Pi_{r,j}, L_{r,j})$, the product transition system  is a tuple $\textup{PTS} = (S^n, s^0, \to, \Pi, L)$ where: (a) $S^n = S\times \cdots \times S$ is the finite set of collective robot locations%% , which requires that no more than one robots occupy the same free cell
; (b) $s^0$ are the initial locations of the robots; (c) $\to \subseteq S^n \times S^n$ is the transition relation so that  $(s, s') \in \to$ if $s_{r,j}\rightarrow_{r,j} s'_{r,j}$ for all $r\in \ccalK_j, \forall \,j \in [m]$;}
  %% Specifically, $(s^t, s^{t+1}) \in \to$ if $s^t_{r,j}\rightarrow_{r,j} s^{t+1}_{r,j}$ for all $r\in \ccalK_j, \forall \,j \in [m]$ and there do not exist any two robots $[r,j]$ and $[r',j']$ such that $s^{t+1}_{r,j} = s^{t}_{r',j'}$ and $s^{t+1}_{r',j'} = s^{t}_{r,j}$. In words, each robot follows its transition relation and no two robots switch their locations;
  (d) $\Pi = \cup_{i\in[|\ccalK_j|], j\in [m], k\in [l]}\{\pi_{i,j}^k\} \cup \{\epsilon\}$, where the atomic proposition $\ap{i}{j}{k}$ is true if  {there exist at least $i$ robots of type $j$}, denoted by $\ag{i}{j}$,  at region $\ell_k$ at the same time, i.e., $\ap{i}{j}{k} \Leftrightarrow |\{r\in \ccalK_j: L_{r,j}(s_{r,j}) = p_{r,j}^k \}| \geq i$; (e) and $L: S^n \to 2^{\Pi}$ is the labeling function.
\end{defn}
\subsection{Task specification}
In this paper, we consider MRTA problems where the task can require the same fleet of robots to visit different regions in sequence, e.g., to deliver objects between different regions. To capture such tasks, we  define {\it induced atomic propositions} over the set $\Pi$ defined in Definition~\ref{def:pts}  as follows.

\begin{defn}[Induced atomic propositions]
   For each basic atomic proposition $\ap{i}{j}{k} \in \Pi$, we define an infinite set of  {induced} atomic propositions $\{\ap{i}{j}{k,\chi}\}_{\chi\in \mathbb{N}}$, where $\chi$ is a connector that binds the truth of  atomic propositions with identical $i, j$ and $\chi$. Specifically, when $\chi=0$, $\ap{i}{j}{k,\chi}$ is equivalent to $\ap{i}{j}{k}$ whose truth is state-dependent. When $\chi \neq 0$, the truth of $\ap{i}{j}{k,\chi}$ is state-and-path-dependent, meaning that it additionally depends on other induced atomic propositions that share the same $i,j$ and $\chi$. That is, both $\ap{i}{j}{k,\chi}$ and $\ap{i}{j}{k',\chi}$  with $\chi\not=0$ are true if  the \textup{same} $i$ robots of type $j$ visit regions $\ell_k$ and $\ell_{k'}$. Furthermore, the negative atomic proposition  $\neg \ap{i}{j}{k,\chi}$ is equivalent to its basic counterpart $\neg \ap{i}{j}{k}$, i.e., less than $\ag{i}{j}$ robots  are at region $\ell_k$.
\end{defn}
Let $\ccalA\ccalP$ collect all basic and induced atomic propositions and  denote by $\Sigma=2^{\ccalA\ccalP}$, its power set.  In what follows, we omit the superscript $\chi$ when $\chi=0$. We denote by {LTL}${^\chi}$, the set of formulas defined over the set of basic and  induced atomic propositions and by {LTL}$^0$, the set of formulas defined only over basic atomic propositions, respectively. Clearly, \ltlx$\supset$ {LTL}$^0$, which means that {LTL}${^\chi}$ can capture a broader class of tasks. {While there exists literature on feasible control synthesis over \ltlz~\citep{sahin2017synchronous,sahin2019multirobot}, to the best of our knowledge there is no work on optimal control synthesis over~\ltlx formulas.} Next, we introduce the notion of {\it valid} temporal logic tasks.
 \begin{defn}[Valid temporal logic task]\label{defn:valid}
A temporal logic task specified by a\ltlx formula defined over $\ccalA\ccalP$ is {\em valid} if atomic propositions with the same nonzero connector $\chi$ involve the same number of robots of the same type.
 \end{defn}
 
\begin{figure}[!t]
\centering
\includegraphics[width=0.35\linewidth]{workspace.pdf}
\caption{Illustration of the workspace for Example~\ref{exmp:1}.}\label{fig:workspace}
\end{figure}

\begin{exmp}[Valid temporal logic tasks]\label{exmp:1}
  {Consider a mail delivery task amidst the COVID-19 pandemic (shown in Fig.~\ref{fig:workspace}) {where three robots of type 1 (green stars) and two robots of type 2 (blue circles) are located at region $\ell_0$ and $\ell_1$, respectively,} $\ell_2$ is an office building that the robots visit to pick up the mail, $\ell_3$ and $\ell_5$ are delivery sites, and $\ell_4$ is a control room from where robots are guided to  the orange area to get disinfected and then drop  off the mail at the delivery site $\ell_3$.  Consider two delivery tasks: {(i)} \label{task:i} Two robots of type 1 visit building $\ell_2$ to collaboratively pick up  the mail  and deliver it to the delivery site $\ell_3$, and one robot of type 2 must visit the control room $\ell_4$ to disinfect robots of type 1  before they get to  the delivery site $\ell_3$. {\it (ii)} \label{task:ii} One robot of type 1 travels between  building $\ell_2$ and the delivery site $\ell_3$ back and forth to transport  equipment, assuming that the disinfection area operates automatically after task \hyperref[task:i]{(i)}.  {Observe that in Fig.~\ref{fig:workspace}, the  atomic propositions satisfied by initial robot locations  are $\ap{3}{1}{0}$ and $\ap{2}{2}{1}$.} }  Tasks \hyperref[task:i]{(i)} and \hyperref[task:ii]{(ii)} can be captured by the valid formulas  $\phi_1 = \lozenge ((\ap{2}{1}{2,1}\wedge \neg \ap{2}{1}{3}) \wedge  \lozenge \ap{2}{1}{3,1})  \wedge \lozenge \ap{1}{2}{4} \wedge \neg \ap{2}{1}{3} \,\mathcal{U}\, \ap{1}{2}{4}$ and $ \phi_2 = \square \lozenge (\ap{1}{1}{2,1} \wedge \lozenge \ap{1}{1}{3,1})$. Note that when binding two atomic propositions, the value of $\chi$ is immaterial as long as it is the same non-zero number. Therefore, $\phi_2$ can also be written as $\square \lozenge (\ap{1}{1}{2,2} \wedge \lozenge \ap{1}{1}{3,2})$.
 However, both formulas $\lozenge (\ap{1}{1}{2,1} \wedge \lozenge \ap{2}{1}{3,1})$ and $\lozenge (\ap{2}{2}{2,1} \wedge \lozenge \ap{2}{1}{3,1})$ are  invalid  as they connect different numbers of robots $i$ and robot types $j$, respectively.
 \end{exmp}
{Let $s^t$ be the collective state at time $t$.} A  path of length $h$ is defined as $\tau = s^0 \ldots s^h$ and it captures the collective behavior of the team  such that $s^{t-1}\to s^{t}, \forall t\in[h]$. {Given a valid LTL$^\chi$ formula $\phi$, a  path $\tau=\tau^{\text{pre}}[\tau^{\text{suf}}]^\omega$ in a prefix-suffix structure that satisfies $\phi$ exists since there exists an accepting run in prefix-suffix form}, where the prefix part  $\tau^{\text{pre}}=s^0 \dots s^{h_1}$ is executed once followed by the indefinite execution of the suffix part $\tau^{\text{suf}}=s^{h_1} \dots s^{h_1+h_2} s^{h_1+h_2+1}$, where $s^{h_1+h_2+1}=s^{h_1}$ \citep{baier2008principles}. We say that a path $\tau$ satisfies $\phi$ if (a) the trace, defined as $\texttt{trace}(\tau):=L(s^0)\dots L(s^{h_1})[L(s^{h_1})\dots L(s^{h_1+h_2+1})]^{\omega}$,  belongs to $\texttt{Words}(\phi^0)$, where $\phi^0$ is obtained by replacing all induced atomic propositions in $\phi$ by  their counterparts with the zero connector and (b) it is the same $\ag{i}{j}$ that satisfy the induced atomic propositions $\ap{i}{j}{k,\chi}$ in $\phi$ sharing the same nonzero connector $\chi$.
% In other words, condition (a) restricts  the label of the path, while condition (b) restricts the robots that participate in the satisfaction of induced atomic propositions. If $\phi \in \textup{LTL}^0$, the satisfaction conditions only include (a).

\subsection{Problem definition}
Given a  path $\tau_{r,j} = s_{r,j}^0, s_{r,j}^1, \ldots, s_{r,j}^h$ of length $h$ for robot $[r,j]$, we define the cost of $\tau_{r,j}$  as $J(\tau_{r,j}) = \sum_{t=0}^{h-1} d(s_{r,j}^{t}, s_{r,j}^{t+1})$, where {$d: S\times S \to \mathbb{R}^+\cup\{0\}$ is a cost function that maps a pair of free cells to a non-negative value, for instance, travel distance or time.} The cost of path $\tau$ that combines all robot paths $\tau_{r,j}$ of length $h$ is given by
\begin{align}
  J(\tau) = \sum_{{r \in \ccalK_j, j \in [m]}} J(\tau_{r,j}).
\end{align}
For  plans written in prefix-suffix form, we get
\begin{align}\label{eq:cost}
J(\tau) = \beta J(\tau^{\text{pre}}) + (1-\beta) J(\tau^{\text{suf}}),
\end{align}
where $\beta\in [0,1]$ is a user-specified parameter. Then,  the problem addressed in this paper can be  formulated as follows.
\begin{problem}\label{prob:1}
  Consider  a discrete workspace with labeled regions and obstacles, a team of $n$ robots of $m$ types, and a valid formula $\phi\in \textit{LTL}^\chi$. Plan a path for each robot such that the specification $\phi$ is satisfied and the cost in~\eqref{eq:cost} is minimized.
\end{problem}

We refer to Problem~\ref{prob:1} as the Multi-Robot Task Allocation problem  under LTL specifications or LTL-MRTA. This is a single-task robot and multi-robot task (ST-MR) problem, where a robot is capable of one task and a task may require multiple robots. Since the ST-MR problem is NP-hard~\citep{nunes2017taxonomy}, so is the LTL-MRTA problem. Consequently, existing approaches to this problem become intractable  for large-scale applications \citep{sahin2017synchronous}. In this work, we propose a new hierarchical  framework  to solve LTL-MRTA problems efficiently.

\subsection{Assumptions}\label{sec:asmp}
In this section, we  discuss  assumptions on the workspace and the  NBA translated from the LTL specifications   that are necessary to ensure completeness of our proposed method. \subsubsection{Workspace}
 The following assumption ensures that regions are  well-defined and mutually exclusive.
 \begin{asmp}[Workspace]\label{asmp:env}
 Regions are disjoint, and each region  spans consecutive cells. There exists a label-free path between any two regions, between any two label-free cells, and between any label-free cells and any regions.
 \end{asmp}
If regions are overlapping or span multiple clusters of cells, we can define additional atomic propositions to satisfy Assumption~\ref{asmp:env}.  Assumption~\ref{asmp:env} implies that there are no ``holes'' inside regions that generate different labels, label-free cells are connected, and each region is adjacent to a label-free cell.

\subsubsection{Nondeterministic B$\ddot{\text{u}}$chi Automaton (NBA)}\label{sec:nba}
Given a team of $n$ robots and an \ltlx formula $\phi$, we can find a path $\tau$ that satisfies $\phi$ by operating  on the corresponding NBA $\autop = (\ccalV, \ccalE)$, which can be constructed using existing  tools, such as LTL2BA developed by~\cite{gastin2001fast}; see also Fig.~\ref{fig:nba_iii} for the NBA of tasks~\hyperref[task:i]{(i)} and~\hyperref[task:ii]{(ii)}. Note that the NBA is essentially a graph. Thus, in the remainder of this paper, we refer to the NBA by the graph $\autop$. Before discussing assumptions on the NBA $\ccalA_\phi$, we present a list of pre-processing steps to obtain an ``equivalent" NBA that does not lose any feasible paths that satisfy the specification $\phi$. {The goal is to remove infeasible and redundant transitions in the NBA to reduce its size.}

Let the propositional formula $\gamma$ associated with a transition $v_1 \xrightarrow{\gamma} v_2$ in the NBA $\autop$ be in {\it disjunctive normal form} (DNF), i.e,
$ \gamma = \bigvee_{p\in \ccalP} \bigwedge_{q\in \ccalQ_p} (\neg)\ap{i}{j}{k,\chi}$, where the negation operator can only precede the atomic propositions and $\ccalP$ and $\ccalQ_p$ are proper index sets. Note that any propositional formula has an equivalent DNF~\citep{baier2008principles}. We call  $\ccalC_p^{\gamma}=\bigwedge_{q\in \ccalQ_p}(\neg) \ap{i}{j}{k,\chi}$ the $p$-th {\it clause} of $\gamma$ that includes a set $\ccalQ_p$ of positive and negative {\it literals} and each positive literal is an atomic proposition $\ap{i}{j}{k,\chi}\in \ccalA\ccalP$. Let $\mathsf{cls}(\gamma)$ denote the set of clauses in $\gamma$. Let $\mathsf{lits}^+(\ccalC_p^{\gamma})$ and $\mathsf{lits}^-(\ccalC_p^{\gamma})$ be the {\it positive subformula} and {\it negative  subformula}, consisting of all positive and  negative literals in the clause $\ccalC_p^\gamma$. Those subformulas are $\top$ (constant true) if the corresponding literals do not exist. In what follows, we do not consider self-loops when we refer to edges in $\autop$, since self-loops can be captured by vertices. We call the propositional formula $\gamma$ a {\it vertex label} if $v_1=v_2$, otherwise, an {\it edge label}.  With a slight abuse of notation, let {$\gamma: \ccalV \to \Sigma $} and {$\gamma: \ccalV \times \ccalV \to \Sigma$} be the functions that map a vertex and edge to its vertex label and edge label, respectively. Given an edge $(v_1, v_2)$, we call labels $\gamma(v_1)$ and $\gamma(v_2)$ the {\it starting} and {\it end} vertex labels, respectively. Next, we  pre-process the NBA $\autop$ by removing infeasible clauses and merging redundant literals.  Consider a vertex  or edge label $\gamma$ in $\autop$, 

\mysubparagraph{Absorption in $\mathsf{lits}^+(\cp{p}{\gamma})$}{For each clause $\cp{p}{\gamma} \in \clause{\gamma}$, we delete the positive literal $\ap{i}{j}{k} \in \mathsf{lits}^+(\cp{p}{\gamma})$, replacing it with $\top$, if another $\ap{i'}{j}{k,\chi'} \in \mathsf{lits}^+(\cp{p}{\gamma})$ exists such that $i \leq i'$.  This is because  if $\ag{i'}{j}$ are at region $\ell_k$, i.e., $\ap{i'}{j}{k,\chi'}$ is true, so is  $\ap{i}{j}{k}$. Similarly, we replace $\ap{i}{j}{k}$ by $\ap{i-i'}{j}{k}$ if $i > i'$, {since $i-i'$ additional robots are needed to make $\ap{i}{j}{k}$ true if  $\ap{i'}{j}{k,\chi'}$ is true.}\label{prune:absorption1}}

\mysubparagraph{Absorption in $\mathsf{lits}^-(\cp{p}{\gamma})$} {We delete the negative literal $\neg \ap{i}{j}{k} \in \mathsf{lits}^-(\cp{p}{\gamma})$, if another $\neg \ap{i'}{j}{k} \in \mathsf{lits}^-(\cp{p}{\gamma})$ exists such that $i' < i$. This is because if $\neg \ap{i'}{j}{k}$ is true, so is $\neg \ap{i}{j}{k}$.}\label{prune:absorption2}

\mysubparagraph{Mutual exclusion in $\mathsf{lits}^+(\cp{p}{\gamma})$}{We delete the clause $\cp{p}{\gamma} \in \mathsf{cls}(\gamma)$, replacing it with constant false $\bot$, if there exist two positive literals $\ap{i}{j}{k,\chi}, \ap{i}{j}{k',\chi} \in \mathsf{lits}^+(\cp{p}{\gamma})$ such that $k\not= k'$ and $\chi\not=0$. The reason is that  the same $i$ robots of type $j$  cannot be at different regions at the same time.} \label{prune:exclusion1}

\mysubparagraph{Mutual exclusion in $\mathsf{lits}^+(\cp{p}{\gamma})$  and $\mathsf{lits}^-(\cp{p}{\gamma})$} { We delete the clause $\cp{p}{\gamma} \in \mathsf{cls}(\gamma)$  {if there exists a positive literal} $\ap{i}{j}{k,\chi} \in \mathsf{lits}^+(\cp{p}{\gamma})$ and a negative literal $\neg \ap{i'}{j}{k} \in \mathsf{lits}^-(\cp{p}{\gamma})$ such that $i' \leq i$. This is because these literals   are mutually  exclusive.} \label{prune:exclusion2}

\mysubparagraph{Violation of team size} {For each clause $\cp{p}{\gamma} \in \clause{\gamma}$, let $\mathsf{lits}^+(j')$ denote literals in $\mathsf{lits}^+(\cp{p}{\gamma})$ that involve robots of type $j'$, i.e., $\mathsf{lits}^+(j') = \{\ap{i}{j}{k,\chi} \in \mathsf{lits}^+(\ccalC_p^\gamma)| j = j'\}$. We delete the clause $\cp{p}{\gamma}$   if the total required number of robots of type $j$ exceeds the size $|\ccalK_j|$, i.e., if there exists $j\in[m]$ such that $ \sum_{\ap{i}{j}{k,\chi}\in\mathsf{lits}^+(j)}   i > |\ccalK_{j}|$.} \label{prune:violation1}

 Note that these pre-processing steps do not  compromise any accepting words in $\ccalL(\autop)$ that can be generated by a feasible path. With a slight abuse of notation, we continue to use $\autop$ to refer to the NBA  obtained  after these pre-processing steps.


Consider an edge $e = (v_1, v_2) $  and its starting vertex $v_1$ in $\autop$ and assume that the current state of $\ccalA_\phi$ is vertex $v_1$. To transition to  $v_2$, certain robots need to simultaneously reach certain regions  or avoid certain regions in order to make $\gamma(v_1, v_2)$ true, while maintaining  $\gamma(v_1)$ true en route. We assume that the transition to $v_2$ occurs immediately once $\gamma(v_1, v_2)$ becomes true. Therefore, we can define by a {\em subtask} the set of actions that need to be taken by robots in order to activate a transition in the NBA. 
\begin{defn}[Subtask]\label{defn:subtask}
  Given an edge $(v_1, v_2)$ in the NBA $\ccalA_\phi$, a subtask is defined by the associated  edge label $\gamma(v_1, v_2)$ and  starting vertex label $\gamma(v_1)$.
\end{defn}

Subtasks can be viewed as generalized reach-avoid tasks where robots visit or avoid certain regions (the ``reach'' part) while satisfying the starting vertex labels along the way (the ``avoid'' part, which here is  more general than avoiding obstacles). Observe that every accepting run in the NBA consists of a sequence of subtasks. However, not all sequences of subtasks are feasible. In what follows, we restrict the accepting runs to those that can complete the task by first  providing insights using the following example.

\begin{figure}[!t]
   \centering
   \subfigure[NBA $\autop$ for the task {(i)}]{
     \label{fig:nba_i}
     \includegraphics[width=0.55\linewidth]{nba_i.pdf}}
   \subfigure[NBA $\autop$ for the task {(ii)}]{
     \label{fig:nba_ii}
     \includegraphics[width=0.4\linewidth]{nba_ii.pdf}}
   \caption{NBA $\autop$ for tasks \hyperref[task:i]{(i)} and \hyperref[task:ii]{(ii)}, {where self-loops are omitted and the corresponding vertex labels are placed in square brackets.}}
   \label{fig:nba_iii}
\end{figure}

 \begin{cexmp}{exmp:1}{Subtasks}\label{exmp:observation}
   The NBAs for  tasks \hyperref[task:i]{(i)} and \hyperref[task:ii]{(ii)} before pre-processing are shown in Fig.~\ref{fig:nba_iii}. After pre-processing, the NBA $\autop$ for task~\hyperref[task:i]{(i)} does not change whereas some labels (orange color) in the NBA $\autop$ for task \hyperref[task:ii]{(ii)} become $\bot$ due to step~\hyperref[prune:exclusion1]{\it (3)}. 
   In Fig.~\ref{fig:nba_i}, $\vertex{init}$ is the initial vertex and $v_6$ is the accepting vertex. Observe that all vertices have self-loops except for the initial vertex $\vertex{init}$. In each accepting run, e.g., $\vertex{init}, v_1, v_2, v_3, v_6, v_6^\omega$, the satisfaction of an edge label leads to the satisfaction of its end vertex label, assuming this end vertex label is not  $\bot$. For instance,  label $\ap{2}{1}{2,1} \wedge \neg\ap{2}{1}{3}$ of  edge $(v_1, v_2)$ implies  label $\neg\ap{2}{1}{3}$ of vertex $v_2$, and  label $\neg\ap{2}{1}{3}$ of edge  $(\vertex{init}, v_1)$ implies  label $\neg\ap{2}{1}{3}$ of  its end vertex $v_1$. Intuitively, the completion of a subtask indicated by the satisfaction of its edge label, automatically activates the subtasks that immediately follow it indicated by the satisfaction of their starting vertex labels. This is because once the edge is enabled, its end vertex label should be satisfied at the next time instant; otherwise, progress  in the NBA $\autop$ will  get stuck. The same observation also applies to the NBA in Fig.~\ref{fig:nba_ii} where the vertex $\vertex{init}$ is both an initial and accepting vertex and $v_3$ is another accepting vertex.  The accepting run $\vertex{init}, v_2, v_3, (v_1, v_2, v_3)^\omega$ includes one pair of initial and accepting vertices, $\vertex{init}$ and  $v_3$, and the accepting run $\vertex{init}, v_2, v_1, \vertex{init}^\omega$ (although infeasible) includes one pair of initial and accepting vertices, $\vertex{init}$ and $\vertex{init}$. Note that we view the two $\vertex{init}$ vertices differently, one as the initial vertex and the other as the accepting vertex. Furthermore, label $\ap{1}{1}{3,1}$ of edge $(v_1, v_2)$  implies  label $\top$ of its end vertex $v_2$; the same holds for the edge $(v_2, \vertex{init})$ and its end vertex $\vertex{init}$ (although infeasible). It is noteworthy that even though the accepting vertex $v_3$ does not have a self-loop, the satisfaction of the label $\ap{1}{1}{2,1}$ of its incoming edge $(v_2, v_3)$ leads to the satisfaction of the label $\top$ of its outgoing edge $(v_3, v_1)$. If the satisfaction of the incoming edge label does not imply satisfaction of the outgoing edge label, then progress in the NBA  will get stuck at $v_3$ since the label $\ap{1}{1}{2,1} \wedge \ap{1}{1}{3,1}$ of edge $(v_3, \vertex{init})$ is infeasible and the transition between regions $\ell_2$ and $\ell_3$ requires more than one time steps; see Fig.~\ref{fig:workspace}, which makes the label $\ap{1}{1}{3,1}$ of edge $(v_3, v_2)$ unsatisfiable at the next time instant.
 \end{cexmp}


 Motivated by the observations in Example~\ref{exmp:1}, we introduce the notions of {\it implication} and {\it strong implication} between two propositional formulas. Then, we define a {\it restricted accepting run} in the NBA $\autop$   in a prefix-suffix structure. The completeness of our method relies on the assumption that the set of restricted accepting runs in the  NBA $\autop$ is nonempty.

 \begin{defn}[Implication and strong implication]\label{defn:implication}
   Given two propositional formulas $\gamma$ and $\gamma'$ over $\ccalA\ccalP$, we say that formula  $\gamma$ implies $\gamma'$, denoted by $\gamma \simplies \gamma'$, if for each clause $\ccalC_{p}^{\gamma} \in \clause{\gamma}$, there exists a clause $\ccalC_{p'}^{\gamma'} \in \clause{\gamma'}$ such that  $\ccalC_{p'}^{\gamma'}$ is a subformula of $\ccalC_{p}^{\gamma}$, i.e., all literals in $\ccalC_{p'}^{\gamma'}$ also appear in $\ccalC_{p}^{\gamma}$. By default, $\top$ is a subformula of any clause. In addition, formula $\gamma$ strongly implies $\gamma'$, denoted by $\gamma \simplies_s  \gamma'$, if $\gamma \simplies \gamma'$, and for each clause $\ccalC_{p'}^{\gamma'} \in \clause{\gamma'}$, there exists a clause $\ccalC_{p}^{\gamma} \in \clause{\gamma}$ such that  $\ccalC_{p'}^{\gamma'}$ is a subformula of $\ccalC_{p}^{\gamma}$.
 \end{defn}

 Intuitively, if $\gamma \simplies \gamma'$ or $\gamma \simplies_s \gamma'$, robot locations that satisfy $\gamma$ also  satisfy  $\gamma'$.

\begin{figure}[t]
  \centering
  \includegraphics[width=0.45\linewidth]{lasso.pdf}
  \caption{Graphical depiction of the accepting run in the prefix-suffix structure when $\vertex{accept}$ does not have a self-loop. The shaded blue line and the orange loop represent the prefix and suffix part, respectively. The arrow indicates the progression direction and the gray circles indicate the self-loops.}
  \label{fig:lasso}
\end{figure}


\begin{defn}[Restricted accepting run]\label{defn:run}
  Given the pre-processed NBA $\autop$  corresponding to an \ltlx formula, we call any accepting run in a  prefix-suffix structure $\rho = \rho^{\textup{pre}} [\rho^{\textup{suf}}]^\omega= v_0, \ldots, \vertex{prior}, \vertex{accept} [\vertex{next}, \ldots, \vertex{prior}', \vertex{accept}]^\omega$ (see Fig.~\ref{fig:lasso}), a restricted accepting run,  if it  satisfies conditions:
  \begin{noindlist}
    \setlength\itemsep{0em}
  \item \label{cond:a} If a vertex is both an initial vertex $v_0 $ and an accepting vertex $\vertex{accept}$, we treat it as two different vertices, namely  an initial vertex and an accepting vertex. The accepting vertex $\vertex{accept}$ appears only once at the end in both the prefix and suffix parts. In the prefix part  $v_0, \ldots, \vertex{prior}, \vertex{accept}$, if a vertex appears multiple times,  all repetitive occurrences are consecutive.  The same holds for  the suffix part  $\vertex{next}, \ldots, \vertex{prior}', \vertex{accept}$;
  \item \label{cond:b} There only exist one initial vertex $v_0$ and one  accepting vertex $\vertex{accept}$ in the accepting run (they can appear multiple times in a row). Different  accepting runs can have different pairs of initial and accepting vertices;
  \item \label{cond:c} In the prefix part, only initial and accepting vertices, $v_0$ and $\vertex{accept}$, are allowed not to have  self-loops, i.e., their vertex labels  can be $\bot$. In the suffix part,  only the accepting vertex $\vertex{accept}$ is allowed not to have a self-loop;
  \item  \label{cond:d} For any two consecutive vertices $v_1$, $v_2$ in the accepting run $\rho$, if $v_1 \neq v_2$, $v_2\neq \vertex{accept}$ and $v_2$ has a self-loop, then the edge label $\gamma(v_1, v_2)$  strongly implies  the end vertex label $\gamma(v_2)$, i.e., $\gamma(v_1, v_2) \simplies_s \gamma(v_2)$;
   %% \item \label{cond:e} For any three consecutive vertices $v_1, v_2$ and $v_3$ in the accepting run, if $v_2 \neq v_{\vertex{accept}}$ and $v_2$ has a self-loop, then either $v_1 = v_2$ or $v_2 = v_3$, that is, the label of  vertex $v_2$ should be satisfied at least once;
   \item \label{cond:e} In the suffix part $\rho^{\textup{suf}}$, if $\vertex{accept} = \vertex{next}$ (this happens when $\vertex{accept}$ has a self-loop), then $\rho^{\textup{suf}}$ only contains the vertex   $\vertex{accept}$. Meanwhile, the label of the edge $(\vertex{prior}, \vertex{accept})$  implies the label of the vertex $\vertex{accept}$, i.e., $\gamma(\vertex{prior}, \vertex{accept}) \simplies  \gamma(\vertex{accept})$;
 \item \label{cond:f} In the suffix part, if $\vertex{accept} \neq \vertex{next}$ (this can happen when $\vertex{accept}$  does not have a self-loop), then the label of the edge $(\vertex{prior}, \vertex{accept})$ implies the label of the edge $(\vertex{accept}, \vertex{next})$, i.e., $\gamma(\vertex{prior}, \vertex{accept}) \simplies  \gamma(\vertex{accept}, \vertex{next})$. Also, the label $\gamma(\vertex{prior}, \vertex{accept})$ implies the label of the  edge $(\vertex{prior}', \vertex{accept})$, i.e., $\gamma(\vertex{prior}, \vertex{accept}) \simplies  \gamma(\vertex{prior}', \vertex{accept})$. Note that $\vertex{prior}$ and $\vertex{prior}'$ can be different.
  \end{noindlist}
 \end{defn}
%\begin{figure*}[!t]
%   \centering
%\includegraphics[width=0.9\linewidth]{overview.pdf}
%   \caption{Schematic overview of the proposed method.  The first five boxes correspond to the relaxation stage and the last two constitute the correction stage.}
%\label{fig:overview}
%\end{figure*}

In what follows, we discuss the conditions in Definition~\ref{defn:run} in more detail. {Specifically, conditions~\ref{cond:a} and~\ref{cond:b} require that a restricted accepting run is  ``simple''.  Specifically, condition~\ref{cond:a} states that vertices  $v_0$ and $\vertex{accept}$ can be treated differently since they mark different progress towards accomplishing a task. The prefix and suffix parts of a restricted accepting run  end once  $\vertex{accept}$ is reached, as in~\cite{smith2010optimal}. By aggregating consecutive identical vertices in the prefix part of  a restricted accepting run into one single vertex,  there are no identical vertices in the ``compressed'' prefix part. That is,  it contains no cycles. The presence of a cycle is redundant since it implies negative progress towards accomplishing the task.  The same applies to the suffix part.}  On the other hand,  condition~\ref{cond:b} states that a restricted accepting run is basically an accepting run defined in Section~\ref{sec:ltl} that is further defined over a pair of initial and accepting vertices. In Section~\ref{sec:app}, we extract smaller sub-NBAs from the NBA $\autop$ for each pair of initial and accepting vertices, which helps reduce complexity of the problem.

Conditions~\ref{cond:c}-\ref{cond:f} require that  the completion of a subtask in a restricted accepting run   automatically activates the subtasks that immediately follow it; see Example~\ref{exmp:1}. This ensures that robots are given adequate time to undertake subsequent subtasks after completing the current subtask. Accepting runs that do not satisfy conditions \ref{cond:c}-\ref{cond:d} are disregarded. In fact, in Section~\ref{sec:prune} we prune vertices and edges in the NBA that violate these conditions, further reducing the size of the NBA.  Finally, the implication $\gamma(\vertex{prior}, \vertex{accept}) \simplies  \gamma(\vertex{accept}, \vertex{next})$ in condition~\ref{cond:f}  requires that the robot locations enabling the last edge in the prefix part of a restricted accepting run  also enable the first edge in the suffix part. As a result, we can find the prefix and suffix parts of a restricted accepting run separately. Otherwise, the progress in the NBA $\autop$  may get stuck since these two edge labels need to be satisfied at two consecutive time instants, similar to conditions~\ref{cond:d} and \ref{cond:e}. Also, as the suffix part of a restricted accepting run  is a loop, robots need to return to their initial locations in the suffix part after executing the suffix part once. The relation $\gamma(\vertex{prior}, \vertex{accept}) \simplies  \gamma(\vertex{prior}', \vertex{accept})$ requires  that the  initial locations in the suffix part of a restricted accepting run  enable the edge  $(\vertex{prior}', \vertex{accept})$, which ensures that the robots can travel back to the initial locations in the suffix part and, as a result, activate  the transition in  $\autop$ back to the vertex $\vertex{accept}$ that allows to repeat the suffix part $\rho^{\text{suf}}$. Finally, we make the following assumption on the structure of the NBA $\ccalA_\phi$.

\begin{asmp}[Existence of restricted accepting runs]\label{asmp:run}
  The set of restricted accepting runs is non-empty.
\end{asmp}

{We note that the sets of restricted accepting runs for tasks~\hyperref[task:i]{(i)} and~\hyperref[task:ii]{(ii)} satisfy Assumption~\ref{asmp:run}. Common robotic tasks, such as sequencing and coverage, have NBAs that contain restricted accepting runs. However, there is also a small subclass of LTL where the ``next"  operator  directly precedes an atomic proposition that violates this assumption. For instance, $\lozenge (\pi_{1,1}^{2,1} \wedge \bigcirc \pi_{1,2}^{3,1})$ requires a second  robot to visit region $\ell_3$ immediately after the first robot reaches $\ell_2$, which does not allow for any physical time between the completion of the two consecutive subtasks. On the other hand, the LTL formula $\lozenge (\pi_{1,1}^{2,1} \wedge \bigcirc (\pi_{1,1}^{2,1} \mathcal{U} \pi_{2,1}^3))$ satisfies the assumption.}
%% Moreover, condition \ref{cond:e} is similar to~\ref{cond:d} in the sense that  the satisfaction of the edge label $\gamma(v_1, v_2)$ leads to the  satisfaction of the end vertex label $\gamma(v_2)$ since the end vertex label needs to be satisfied immediately after the edge label.
%% In Sections~\ref{sec:app} and~\ref{sec:solution}, we first consider a relaxed NBA where all negative literals are ignored, and then re-consider negative literals in Section~\ref{sec:solution2mrta}. The conditions \ref{cond:d} and \ref{cond:e} ensure that the plan obtained by only considering the positive subformulas can be modified to accommodate the ignored negative subformula.
    %%  In Appendix~\ref{sec:discussion}, we will discuss the relaxation of strong implication to implication.
      %% by preventing the mutual exclusions between positive and negative subformulas.



\subsubsection{Robot paths}
      The definition of restricted  accepting runs is based entirely on the structure of the  NBA and logical implication relations. However, Definition~\ref{defn:run} does not describe how to characterize robot paths that induce restricted accepting runs. Next, we discuss conditions under which robot paths satisfy restricted accepting runs. We call such paths {\em satisfying paths} and we assume such satisfying paths exist.


\begin{defn}[Satisfying paths of restricted accepting runs]\label{defn:same}
  Given a team of $n$ robots and a valid specification $\phi \in \textit{LTL}^\chi$, a robot path $\tau$ is a satisfying path that induces a restricted accepting run, if the following conditions hold:
  \begin{noindlist}
  \item \label{asmp:a} If a vertex label is satisfied by the path $\tau$, it is always satisfied by the same clause that is always satisfied by the same fleet of robots;
  \item  \label{asmp:b} If a clause in an edge label is satisfied by the path $\tau$, then a clause in the end vertex label is also satisfied. Moreover, the fleet of robots satisfying the positive subformula of the clause in the end vertex label is the same as the fleet of robots satisfying the positive  subformula of the clause in the corresponding edge label;
    %% (c)\label{asmp:c} the fleet of robots that satisfy the positive subformula in certain clause of the edge $(\vertex{prior}, \vertex{accept})$ in the prefix part returns to their respective regions when the label of the edge $(\vertex{prior}', \vertex{accept})$ is satisfied in the suffix part.
    \item \label{asmp:c} Robot locations  enabling the edges $(\vertex{accept}, \vertex{next})$ and  $(\vertex{prior}', \vertex{accept})$ in the suffix part of a restricted accepting run  are identical to robot locations enabling the  edge $(\vertex{prior}, \vertex{accept})$ in the prefix part.
  \end{noindlist}
\end{defn}

Definition~\ref{defn:same} is closely related to the definition of a restricted accepting run. Specifically, condition~\ref{asmp:a} in Definition~\ref{defn:same} requires that once a fleet of robots satisfies a vertex label in a restricted accepting run, then these robots remain idle during the next time instant so that the same clause in this vertex label is still satisfied. This satisfies condition~\ref{cond:a} in Definition~\ref{defn:run}. Furthermore, condition~\hyperref[asmp:b]{(b)} in Definition~\ref{defn:same} requires that once a fleet of robots satisfies an edge label in a restricted accepting run, then these robots remain idle during the next time instant so that the clause in the end vertex label that is implied by the clause that is satisfied in the edge label is also satisfied. This satisfies condition~\ref{cond:d} in Definition~\ref{defn:run}.

Finally, condition~\hyperref[asmp:c]{(c)}  in Definition~\ref{defn:same} requires that the robot locations  enabling the edge $(\vertex{prior}, \vertex{accept})$ in the prefix part of a restricted accepting run coincide with the initial locations of the robots that enable the edge  $(\vertex{prior}', \vertex{accept})$ in the suffix part of the restricted accepting run, as per condition~\ref{cond:f} in Definition~\ref{defn:run}. Therefore, condition~\hyperref[asmp:c]{(c)} in Definition~\ref{defn:same} requires that the robots travel along a loop
 so that the suffix part of the restricted accepting run is executed indefinitely. In what follows, we make the following assumption.

\begin{asmp}[Existence of paths]\label{asmp:same}
  Robot paths exist that satisfy the restricted accepting runs in the NBA $\ccalA_\phi$.
\end{asmp}


%% Specifically, by condition~\ref{cond:a} in Definition~\ref{defn:run}, each vertex in a restricted accepting run can only be visited within a consecutive time period.  Once locations of a fleet of robots satisfy a  vertex label, they can remain idle to maintain the satisfaction of the same clause in this vertex label, satisfying condition~\hyperref[asmp:a]{(a)} in Assumption~\ref{defn:same}. Furthermore, by condition~\ref{cond:d} in Definition~\ref{defn:run}, once locations of a fleet of  robots satisfy an edge label, they can remain idle at the next time instant, leading to the satisfaction of the clause in the end vertex label that the satisfied clause in the edge label implies. Thus, condition~\hyperref[asmp:b]{(b)} is  satisfied. As for condition~\hyperref[asmp:c]{(c)}, the robot locations  enabling the edge $(\vertex{prior}, \vertex{accept})$ in the prefix part are the initial locations of the suffix part, which can enable the edge  $(\vertex{prior}', \vertex{accept})$ according to condition~\ref{cond:f} in Definition~\ref{defn:run}. Therefore, condition~\hyperref[asmp:c]{(c)} demands that the robots travel along a loop when advancing the infinite number of repetitions of the suffix part.

%% \subsection{Outline of the LTL-MRTA Algorithm}
%% { \begin{algorithm}[t]
%%       \caption{Outline of the LTL-MRTA Algorithm}
%%       \LinesNumbered
%%       \label{alg:frame}
%%       \KwIn {workspace $\ccalW$,  robot team $\{\ccalK_j\}$\\ \quad \quad \quad
%%        \ltlx formula $\phi$}
%%       Translate $\phi$ into an NBA $B_o$ \label{frame:nba}\Comment*[r]{\ref{sec:prune}}
%%       Prune $B_o$ and do replacing to get $B_r$ \label{frame:prune}\Comment*[r]{\ref{sec:prune}}
%%       Sort pairs of initial and accepting vertices in ascending order by the total length\label{frame:sort} \Comment*[r]{\ref{sec:pregraph}}
%%       \For{each pair in the sorted order}{
%%         \Comment*[r]{Find robot prefix paths}
%%         Extract the sub-NBA $B_s$\ and prune $B_s$ \label{frame:sub-NBA}\Comment*[r]{\ref{sec:pregraph}}
%%         Extract subtasks from $B_s$ and infer the poset with the largest width \label{frame:poset}\Comment*[r]{\ref{sec:poset}}
%%         Build the MILP graph; see also Alg.~\ref{alg:milpgraph} \label{frame:milpgraph}\Comment*[r]{\ref{sec:graph}}
%%         Formulate the MILP and solve it \label{frame:milp} \Comment*[r]{\ref{sec:milp}}
%%         Extract high-level plans  \label{frame:path} \Comment*[r]{\ref{sec:path}}
%%         Identify the accepting run in $B_r$ \label{frame:run} \Comment*[r]{\ref{sec:run}}
%%         Solve generalized  multi-robot path planning to obtain executable paths\label{frame:mapp} \Comment*[r]{\ref{sec:mapp}-\ref{sec:solution2mapp}}
%%         \Comment*[r]{Find robot suffix paths
%%         }
%%         Repeat lines~\ref{frame:sub-NBA}-\ref{frame:mapp} \label{frame:suffix} \Comment*[r]{\ref{sec:suf}}
%%       }
%% Select the plan with the lowest cost according to~\eqref{eq:cost} \label{frame:cost}
%%  \end{algorithm}}
\subsection{Outline of the proposed method}
           {An overview of our proposed method is shown in Alg.~\ref{alg:ltlmrta}, which first finds prefix paths and then suffix paths.  The process of finding prefix or suffix paths consists of relaxation and correction stages. 
             Specifically, during the relaxation stage, we ignore the negative literals in the NBA $\ccalA_\phi$ and formulate a MILP to allocate subtasks to robots and determine time-stamped robot waypoints  that satisfy the task assignment. To this end, we first prune the NBA $\autop$ by deleting infeasible transitions and then relax it by removing negative subformulas  so that transitions in the relaxed NBA are solely satisfied by robots that meet at certain regions [line~\ref{ltl:relax}]; see Section~\ref{sec:prune}. The idea to temporarily remove negative literals from the NBA is motivated by ``lazy collision checking'' methods in robotics and allows to simplify the planning problem as the constraints are not considered during planning and are only checked during execution, when needed. {Then,  since by condition~\ref{cond:b} in Definition~\ref{defn:run}, restricted accepting runs contain  only one initial vertex and one accepting vertex, for every sorted pair of initial and accepting vertices by length in the relaxed NBA, we extract a sub-NBA of smaller size [line~\ref{ltl:prefix}];} see Section~\ref{sec:pregraph}, where $\auto{subtask}(\vertex{init}, \vertex{accept})$ is the sub-NBA including only initial vertex $\vertex{init}$, accept vertex $\vertex{accept}$ and other intermediate vertices. The sub-NBAs are used to extract subtasks and temporal orders between them captured by a set of posets ([lines~\ref{ltl:pruneprefix}-\ref{ltl:inferprefix}], see Section~\ref{sec:poset}), and construct routing graphs, one for each poset,  that capture the regions that the robots need to visit and the temporal order of the visits so that the subtasks extracted from the sub-NBAs are satisfied; see Section~\ref{sec:graph}. Finally, given the routing graph corresponding to each poset we formulate a MILP inspired by the vehicle routing problem to obtain a high-level task allocation plan along with time-stamped waypoints that the robots need to visit to satisfy the task assignment [lines~\ref{ltl:prefixgraph}-\ref{ltl:prefixmilp}]; see Section~\ref{sec:path}. During the correction stage, we introduce the negative literals back into the NBA and formulate a collection of generalized multi-robot path planning problems, one for each poset, to design low-level executable robot paths that satisfy the original specification ([line~\ref{ltl:prefixgmrpp}], see Section~\ref{sec:lowlevel}). Viewing the final states of the prefix paths as the initial states, a similar process is conducted for the sub-NBA $\auto{subtask}(\vertex{accept}, \vertex{accept})$ to find the suffix paths. Alg.~\ref{alg:ltlmrta} can terminate after a specific number of paths is found or all possible alternatives are explored.  Under the mild assumptions discussed in Section~\ref{sec:asmp}, completeness of our proposed method is shown in Theorem~\ref{thm:completeness} in Section~\ref{sec:correctness}.}

 \begin{algorithm}[!t]
       \caption{Algorithm for LTL-MRTA}
       \LinesNumbered
       \label{alg:ltlmrta}
       {
       Prune and relax the NBA \label{ltl:relax}\;
         \ForEach{\textup{sorted sub-NBA} $\auto{subtask}(\vertex{init}, \vertex{accept})$ \label{ltl:prefix}}{
                \Comment*[r]{Compute the prefix path}
         Prune the sub-NBA $\auto{subtask}(\vertex{init}, \vertex{accept})$\label{ltl:pruneprefix}\;
         Infer the set of posets $\{P_{\textup{pre}}\}$\label{ltl:inferprefix}\;
         \ForEach{\textup{sorted poset} $P_{\textup{pre}}$}{
            Build the routing graph \label{ltl:prefixgraph}\;
            Formulate MILP to get prefix high-level plans \label{ltl:prefixmilp}\;
            Formulate generalized multi-robot path planning to get prefix low-level paths \label{ltl:prefixgmrpp}\;
                            \Comment*[r]{Compute the suffix path}
            Prune the sub-NBA $\auto{subtask}(\vertex{accept}, \vertex{accept})$\label{ltl:prunesuffix}\;
                     Infer the set of posets $\{P_{\textup{suf}}\}$\label{ltl:infersuffix}\;
         \ForEach{\textup{sorted poset} $P_{\textup{suf}}$}{
            Build the routing graph\label{ltl:suffixgraph}\;
            Formulate MILP to get suffix high-level plans\label{ltl:suffixmilp}\;
            Formulate generalized multi-robot path planning to get suffix low-level paths\label{ltl:suffixgmrpp}\;
         }
         }}   }
\end{algorithm}  

%% %% %% %% \begin{rem}
%% %% %% %% The proposed method is not limited to  LTL$_{-\bigcirc}^\chi$ formulas. It can also be applied to  formulas that include the ``next'' operator but have a nonempty set of restricted accepting runs, such as $\lozenge\left(\ap{1}{1}{2,1} \wedge \bigcirc \left(\ap{1}{1}{2,1} \,\ccalU\, \ap{1}{2}{2}\right)\right)$ and $\lozenge \left(\ap{1}{1}{2}  \wedge \bigcirc \lozenge \ap{1}{2}{2}\right)$; see Section~\ref{sec:sim} for simulations. Also,
%% \end{rem}

\begin{rem}
%% In practice, the workspace does not necessarily satisfy Assumption~\ref{asmp:env}, as Fig.~\ref{fig:workspace} in Example~\ref{exmp:1} where no label-free paths between regions~$\ell_3$ and $\ell_5$. In Section~\ref{sec:sim}, various specifications are satisfiable using this workspace.
We note that Assumption~\ref{asmp:same} on the existence of satisfying paths is only a sufficient condition  that needs to be satisfied to show completeness of our proposed method, as shown in the theoretical analysis of Section~\ref{sec:correctness}. The robot path returned by our method may not be a satisfying path, although  it still satisfies the specification $\phi$.
\end{rem}

